Adaptive Coding for Matrix Multiplication at Edge Networks

Edge computing is emerging as a new paradigm to allow processing data at the edge of the network, where data is typically generated and collected, by exploiting multiple devices at the edge collectively. However, exploiting the potential of edge computing is challenging mainly due to the heterogeneous and time-varying nature of edge devices. Coded computation, which advocates mixing data in sub-tasks by employing erasure codes and offloading these sub-tasks to other devices for computation, is recently gaining interest, thanks to its higher reliability, smaller delay, and lower communication cost. In this paper, our focus is on characterizing the cost-benefit trade-offs of coded computation for practical edge computing systems, and develop an adaptive coded computation framework. In particular, we focus on matrix multiplication as a computationally intensive task, and develop an adaptive coding for matrix multiplication (ACM^2) algorithm by taking into account the heterogeneous and time varying nature of edge devices. ACM^2 dynamically selects the best coding policy by taking into account the computing time, storage requirements as well as successful decoding probability. We show that ACM^2 improves the task completion delay significantly as compared to existing coded matrix multiplication algorithms.

==> related.tex <==
\section{\label{sec:related} Related Work}

The use of MDS codes for coded computations was recently proposed and studied ~\cite{SpeedUp-journal, SpeedUp-conference} and attracted remarkable interest from the information and communication theory research communities. Significant effort is being put on constructing codes for fast and distributed matrix-vector multiplication \cite{SpeedUp-journal, ferdinand2016anytime}, matrix-matrix multiplication \cite{yu2017polynomial, lee2017high, fahim2017optimal, yu2018straggler}, dot product and convolution of two vectors \cite{dutta2016short, dutta2017coded}, gradient descent \cite{tandon2017gradient, halbawi2018improving, pmlr-v80-raviv18a}, distributed optimization \cite{karakus2017encoded, karakus2017straggler}, Fourier transform \cite{yu2017coded, jeong2018coded}, and linear transformations  \cite{yang2017computing}. 
Furthermore, the trade-off between latency of computation and load of communication for data shuffling in MapReduce framework \cite{dean2008mapreduce} is characterized in \cite{Tradeoff-conference, Tradeoff-journal}, and optimum resource allocation algorithm is developed in \cite{yu2017optimally}. This coding idea is extended for cellular networks \cite{li2017scalable}, multistage computation \cite{li2016coded}, and heterogeneous systems \cite{kiamari2017heterogeneous}. 


Existing solutions for matrix multiplication do not address the full range of challenges unique to edge computing. Specifically, {\em (i) dynamic and heterogeneous nature:} which requires adaptive  algorithms to allocate coded computation tasks while handling heterogeneous and time-varying resources and changing topologies, 


 
